The Price of Anarchy in Large Games

Game-theoretic models relevant for computer science applications usually feature a large number of players. The goal of this paper is to develop an analytical framework for bounding the price of anarchy in such models. We demonstrate the wide applicability of our framework through instantiations for several well-studied models, including simultaneous single-item auctions, greedy combinatorial auctions, and routing games. In all cases, we identify conditions under which the POA of large games is much better than that of worst-case instances. Our results also give new senses in which simple auctions can perform almost as well as optimal ones in realistic settings.

==> auctions.tex <==
% !TEX root=large.tex

%In this section, we apply our framework to study the efficiency of auction mechanisms in the large.  
%\vsdelete{In an auction mechanism, bidders compete for a set of goods.  If the mechanism is truthful, then bidders submit their values as bids in equilibrium and the allocation is efficient in that it maximizes the total value of the bidders.  If the mechanism is not truthful, then this need not be the case.  However, we show that as the market grows in a sense to be specified later, if the mechanism is well-behaved, then each bidder faces a critical price for his allocation that is insensitive to his own bids.  This allows us to bound the inefficiency of the mechanism using our smoothness-in-the-large framework.}\vscomment{Seems intro text and at this point I would be more technical to the point.}



%We formally define a general mechanism $\M^n$ for a fixed market size $n$. For implicity of notation we drop the superscript $n$ in this paragraph, but in general everything we described can be dependent on the market size. A mechanism $\M$ defines a bid or strategy space $S_i$ for each bidder $i\in [n]$ and we denote with $S=S_1\times\ldots\times S_n$.  For any strategy profile $s\in S$ of bidders, the mechanism selects for each player $i$ a (potentially randomized) allocation $x_i(s)\in\{\N^{m}\}^n$ and a payment $\Theta_i(s)$.  An allocation is feasible if, for all goods $j\in[m]$, at most $k_j$ units are allocated, i.e., $\sum_{i=1}^n x_i^{j}(s)\leq k_j$.  The optimal feasible allocation, $\opt(v)$ is the one that maximizes the total value $\sum_{i=1}^n v_i(x_i)$.  A bidder's utility for an allocation is his value minus his payment, i.e., $u_i(s;v_i)=v_i(x_i(s))-\Theta_i(s)$.  The revenue of a mechanism is the sum of the payments, i.e., $\rev(s)=\sum_{i=1}^{n}\Theta_i(s)$. When we talk about a sequence of mechanisms, all the above can be varying with $n$, i.e. $S^n=S_i^n\times\ldots\times S_n^n$, $\{x_i^n\}_{i=1}^{n}$, $\{\Theta_i^n\}_{i=1}^{n}$, $\{k_j^n\}_{j=1}^{m}$, $\opt^n(\cdot)$, $\rev^n(\dot)$. The only fixed constants is $H$, $m$ and $r$.
%
%With these definitions, we can restate our framework from Section~\ref{prelim} in the context of the mechanism setting.
%
%\begin{defn}[Smooth Mechanism in the Large] A sequence of mechanisms $\Mn$ is $(\lambda,\mu)$-smooth in the large if  if for any $\epsilon>0$, there exists $n(\epsilon)<\infty$, such that for any $n>n(\epsilon)$, for any $v^n\in \V^n$, for each $i\in [n]$, there exists a strategy $s_i^{*,n}\in S_i^n$, such that for any $s^n\in S^n$:
%\begin{equation}
%\sum_i u_i^n(s_{i}^{*,n},s_{-i}^n;v_i^n) \geq \lambda (1-\epsilon) \opt^n(v^n) - \mu \rev^n(s^n)
%\end{equation}
%\end{defn}
%
%Essentially, if a mechanism is $(\lambda,\mu)$-smooth in the large, then for any $\epsilon$, for sufficiently large $n$, any mechanism $\M^n$ is a $(\lambda(1-\epsilon),\mu)$-smooth mechanism according to \cite{Syrgkanis2013}. Thereby the $\BNE$-$\poa^n\leq \frac{\max\{1,\mu\}}{\lambda(1-\epsilon)}$. Thus the Bayes-Nash price of anarchy of a $(\lambda,\mu)$-smooth in the large mechanism converges to $\frac{\max\{1,\mu\}}{\lambda}$.
%
%Similarly, to Section \ref{sec:framework} a sequence of mechanisms $\Mn$ is $(\lambda,\mu)$-smooth in the large, if they admit a sequence of $(\lambda,\mu)$-smooth approximate utility functions $\Seq{U}$, such that $U_i^n$ converge uniformly over $i\in [n]$, $s^n\in S^n$ and $v^n \in \V^n$ to the true utility functions $u_i^n$ and if they satisfy a $(\lambda,\mu)$-smoothness property with respect to $\M^n$ for each $n$: for any valuation profile $v^n\in \V^n$, for each $i\in [n]$, there exists a strategy $s_i^{*,n}\in S_i^n$, such that for any strategy profile $s^n\in S^n$:
%\begin{equation}
%\sum_{i=1}^{n} U_i^n(s_i^{*,n},s_{-i}^n;v_i^n) \leq \lambda \opt^n(v^n) -\mu\cdot \rev^n(s^n)
%\end{equation}
%%\begin{defn}[Smooth Approximate Utility for Mechanisms]
%%A sequence of utility functions $U_i^n$ is a smooth approximate utility sequence with respect to a sequence of mechanisms $\M^n$ if:
%%\begin{enumerate}
%%\item {\bf(Approximation)}\label{prop:approximation} The approximate utility $U_i^n$ converges to the true utility. For any valuation functions $v_i$ and sequence of action profiles $a^n$:
%%\begin{equation}
%%\lim_{n\rightarrow \infty} \left\|u_i^n(a^n; v_i) -U_i^n(a^n; v_i)\right\|=0
%%\end{equation}
%%\item {\bf(Smoothness)} For each mechanism in the sequence, the approximate utility satisfies a $(\lambda,\mu)$-smoothness property. For any $n$, for any valuation profiles $v_i$, for each $i\in [n]$, there exists an action $a_i^{*}\in A_i$, such that for any action profile $a\in \A$:
%%\begin{equation}
%%\sum_{i=1}^{n} U_i^n(a_i^{*},a_{-i};v_i) \leq \lambda \opt^n(v) -\mu\cdot \rev^n(a)
%%\end{equation}
%%\end{enumerate}
%%\end{defn}
%
%Under the latter condition and assuming that the optimal welfare increases at the same or higher asymptotic rate as $n$, we get that the mechanism is smooth in the large.
%\begin{theorem}
%If a sequence of mechanisms $\Mn$ admits $(\lambda,\mu)$-smooth approximate utilities and $\opt^n(v)=\Omega(n)$, then the  sequence of mechanisms is $(\lambda,\mu)$-smooth in the large.
%\end{theorem}

%
%\begin{example}[Uniform Price Auction] Consider a uniform price auction with unit-demand bidders: $k$ units of a good are for sale and each bidder wants one unit, having value $v_i$. Each bidder submits a bid $b_i$ and let $b=(b_1,\ldots,b_n)$. The $k$ highest bids are allocated a unit and each person who is allocated a unit pays the highest losing bid, denoted as $\theta_{k+1}(b)$.
%
%Intuitively, as the auction grows large you would expect that there is enough randomness in the market that a player's effect in determining the price $\theta_{k+1}(b)$, vanishes to zero. Hence, as a player consider his utility from any deviation, he might as well not take into account the effect of his bid on the threshold price.
%\begin{equation}\label{eqn:util-decomp-uniform}
%U_i(s_1,\ldots,s_n; v_i) = (v_i - \theta_{k+1}(s_{-i}))\cdot p(s)
%\end{equation}
%where $p(s)$ is the probability of being allocated with a bid of $s_i$. Under the random tie-breaking (i.e. bidders that are tied at the last bid are randomly ordered) this can be written as:
%\begin{equation}
%p(s) ={\bf 1}\{s_i>\theta_{k+1}(s_{-i})\}+{\bf 1}\{s_i=\theta_{k+1}(s_{-i})\}\cdot\frac{k-|\{j\in [n]: s_j>\theta_{k+1}(s_{-i})\}|}{|\{j\in [n]: s_j=\theta_{k+1}(s_{-i})\}|}
%\end{equation}
%In section \ref{sec:uniform} we will show that if there is sufficient noise in the auction, then the latter function is a valid non-atomic delusional utility for the uniform price auction.
%
% Under the decomposition that we defined in the previous section, it is easy to see that the uniform price auction is a non-atomic $(1,1)$-smooth mechanism. For any valuation profile $v\in T^n$ let $x_i^*(v)$ be the indicator variable of whether player $i$ is allocated a unit under the welfare maximizing allocation. Consider the deviating strategy profile $s^*=(v_1,\ldots,v_n)$, i.e. players deviate to bidding truthfully. Then:
%\begin{align*}
%\sum_i U_i^n(v_i,s_{-i}; v_i)\geq~& \sum_i \left(v_i - \theta_{k+1}(s_{-i})\right)\cdot {\bf 1}\{v_i> \theta_{k+1}(s_{-i})\}= \sum_i \left(v_i-\theta_{k+1}(s_{-i})\right)^+\\
%\geq~& \sum_i (v_i-\theta_{k+1}(s_{-i}))\cdot x_i^*(v) \geq \opt(v) - \theta_{k+1}(s) \sum_i x_i^*(v)\\
% \geq~& \opt(v)-\theta_{k+1}(s) \cdot k = \opt(v) -\rev^n(s)
%\end{align*}
%\end{example}

\subsection{Simultaneous Uniform Price Auctions}
\input{simultaneous-uniform.tex}


\subsection{Greedy Combinatorial Auctions}
\input{greedy-combinatorial.tex}



%\subsection{Proportional Bandwidth Allocation}






==> intro_-_old.tex <==
% !TEX root=large.tex

%\section{Smoothness in Large Markets}
\begin{chapquote}{Gul and Postlewaite, 1992, p. 1273}
... while there may be asymmetry in agents' information, it is relatively unimportant for the problem
at hand because any single agent has only a small amount of information not known by the other agents.
\end{chapquote}

When evaluating the performance of a given market, an important consideration is the extent to which it guarantees efficient outcomes.  In other words, to what extent are resources allocated in accordance with minimizing social cost, or maximizing social welfare?  Markets need not be efficient, especially when the market is small or is dominated by a few influential participants.  For instance, XXX.  However, as a market grows larger in size, the effect of each individual player is negligible. Thereby it is natural to expect that the effects of strategic manipulations by each individual player will be alleviated and the worst-case inefficiency of equilibrium outcomes will improve.  

Indeed, for a variety of special cases, market efficiency has been established under large-market conditions.  Such analysis typically proceeds via an explicit description of market equilibrium (or approximate equilibrium), which can be simple in the limit as markets grow large.  For small markets, a recent line of literature in algorithmic game theory has set about to bound the extent of inefficiency at equilibrium.  This latter analysis eschews a full understanding of equilibrium in favor of approximation bounds, typically via the increasingly standard smoothness framework \cite{}.  However, as price of anarchy results hold for arbitrary markets, they do not capture comparisons between markets of different sizes.

We propose a formalization of the intuition that markets become efficient in the large, via the smoothness framework.  We define the notion of \emph{smoothness in the large}, which bounds inefficiency at equilibrium for a sequence of games with a growing set of players.  Our framework unifies many large-market results from the literature, and can be used to establish efficiency in novel contexts.  Moreover, smoothness in the large can be used to analyze large-market games that are not efficient.  We can therefore address questions of the form: \emph{how does the efficiency of a market's outcomes change as a function of its size?}  Since our definition of smoothness provides worst-case guarantees also for markets of finite size, our framework captures the rate at which game outcomes become (more) efficient as the game grows large.

\paragraph{Our framework}

The standard notion of {\it smoothness} bounds the inefficiency of equilibria not by characterizing the set of equilibria, but rather by considering potential strategy deviations.  The idea is that in any equilibrium, by definition, no player should be able to improve his outcome by deviating from his equilibrium strategy.  One can thus bound the quality of the equilibrium outcome by the sum of deviation outcomes.  
By choosing clever deviations related to the optimal allocation, this sum can often then be decomposed into $\lambda$ times a portion relating to the quality of the optimal plus $\mu$ times a portion relating to the quality of the equilibrium.  Such a game is called $(\lambda,\mu)$-smooth, and its price of anarchy (i.e., ratio of worst equilibrium quality to optimal quality) is at most $\lambda/(1+\mu)$.

Inspired by the standard notion of {\it $(\lambda,\mu)$-smoothness} for finite games, we define a sequence of games to be {\it $(\lambda,\mu)$-smooth in the large} if there is a sequence of strategy deviations that allow us to prove $(\lambda(1+\epsilon),\mu)$-smoothness of each finite game for some $\epsilon=o(1)$.  This implies that the game's price of anarchy converges to $\lambda/(1+\mu)$ at a rate of $\epsilon$ as the game grows large.

We offer one canonical approach for proving that games are smooth-in-the-large.  The approach leverages our intuition that the reason large games are more likely to be efficient is because individual players become insignificant and thus can't impact the outcome much.  The approach first defines for each player an {\it approximate utility}.  This is meant to represent the utility a player might receive in the game if he reasons about it incorrectly by assuming his strategy has minimal effect on his utility.\footnote{Note this is purely for the sake of analysis; the resulting bound on the price of anarchy applies with respect to equilibria of the actual game.}  For example, in a routing game, this could be the cost a player experiences if he doesn't count his own flow towards the congestion of the links.  Similarly, in a multi-item auction game, this might be the utility a player would receive if, when changing his bids, the prices of the items remain fixed (note this may or may not be true of the actual auction).  We require that this utility approximates the actual utility arbitrarily well as the game grows large for any fixed strategy profile.  We further require that the approximate utility is  $(\lambda,\mu)$-smooth {\it with respect to the actual game} (i.e., the sum of deviation utilities is bounded by $\lambda$ times a portion relating to the quality of the optimal plus $\mu$ times a portion relating to the quality of the equilibrium computed using the actual utility functions).  Our main proposition states that if a sequence of games admits a smooth approximate utility, and if the quality of the optimal solution grows as the game grows, then the game is $(\lambda,\mu)$-smooth in the large.

\paragraph{Our results}

To illustrate the power of our framework, we provide a number of examples...


\begin{enumerate}
%\item small markets: friction generates inefficiency.  Price of Anarchy analysis gives a way to approach this.  Many examples.  Technique: smoothness.
%\item as market grows large, the effect of individuals becomes negligible.  inefficiency should be alleviated.
%\item we provide a formalization of this intuition via the smoothness framework.  
%\item this has been analyzed in a variety of contexts.  For example: swinkels, budish.  Idea is that, in the large, game is simple enough that equilibrium can be explicitly solved, and is efficient.  Our formalization unifies this analysis, but also applies in circumstances where equilibrium structure of even the large-limit game is not explicitly understood.
%\item We define smoothness in the limit, which is a condition on the payoff structure of the game that must hold in the limit as the game grows large.
%\item The limit smoothness framework also provides worst-case efficiency guarantees for any finite market size.  That is...  (definition).  So our framework also captures the rate at which game outcomes become more efficient as the game grows large.
%\item We give examples to demonstrate the power of our reduction:
%\begin{enumerate}
\item a very general full efficiency result for simultaneous uniform price auctions in a market with many goods and combinatorial valuations. Specifically, we show that if the number of players and the number of units of each good grows and each player doesn't arrive in the market with some small negligible probability and has finite demand from each good, then the resulting mechanism is $(1,1)$-smooth in the limit, and therefore any $\BCCE$ converges to a fully efficient allocation. Our results heavily generalize on previous work on efficiency in large markets \cite{Swinkels2001}, that only considers a single good and decreasing marginal valuations, whilst not providing any approximation guarantee for finite market sizes.
\item the uncertainty in player arrival is necessary: in the absence of noise, or even if the uncertainty is only over the supply, the large-limit market may not reach efficiency.  
\item for congestion games, we apply our framework to establish that price of anarchy degrades gracefully from its atomic PoA to its non-atomic PoA as the number of players grows large.
\item in a single-minded combinatorial auction, we show that under a greedy $c$-approximate allocation rule we obtain PoA of $c$ in the large-market limit.  Specifically, if the number of players and the number of units of each good grows, and there is sufficient uncertainty in the number of copies of each good present, then the resulting mechanism is $(1,c)$-smooth in the limit.
%\end{enumerate}
\end{enumerate}

%As a market grows larger in size, the effect of each individual player is negligible. Thereby it is natural to expect that the effects of strategic manipulations by each individual player will be alleviated and the worst-case inefficiency of equilibrium outcomes will improve.

%We propose a formalization of the above intuition via the smoothness framework. We define the notion of smoothness in the limit: \emph{a mechanism might not be $(\lambda,\mu)$-smooth for any finite size of the market but becomes $(\lambda,\mu)$-smooth in the limit of an infinitely large market.} 

%The limit smoothness framework also provides worst-case efficiency guarantees for any finite market size, i.e. if a mechanism is $(\lambda,\mu)$-smooth in the limit, then for any $\epsilon$, there exists a finite market size, such that the mechanism is $\left(\frac{\lambda}{1+\epsilon},\mu\right)$-smooth and therefore for sufficiently large markets the $\BCCE$-$\poa$ is at most $(1+\epsilon)\frac{\max\{1,\mu\}}{\lambda}$. 
%
%Via the limit smoothness framework we show a very general full efficiency result for simultaneous uniform price auctions in a market with many goods and combinatorial valuations. Specifically, we show that if the number of players and the number of units of each good grows and each player doesn't arrive in the market with some small negligible probability and has finite demand from each good, then the resulting mechanism is $(1,1)$-smooth in the limit, and therefore any $\BCCE$ converges to a fully efficient allocation. Our results heavily generalize on previous work on efficiency in large markets \cite{Swinkels2001}, that only considers a single good and decreasing marginal valuations, whilst not providing any approximation guarantee for finite market sizes.


==> old-single-uniform-proof.tex <==
\paragraph{Uniform Price Auction with Unit-Demands.} 

In the uniform price auction with endogenous demand uncertainty, each player $i$ doesn't arrive with probability $\delta>0$. Thus if we denote with $z_i$ an indicator random variable that is $1$ with probability $1-\delta$ and with $z=(z_1,\ldots,z_n)$, then the utility of a player for any instantiation of these random variables can be written as:
\begin{equation}
u_i^{n,z}(s; v_i) = u_i^{n,\text{UPA}}(s\cdot z; v_i)\cdot z_i
\end{equation}
where $u_i^{n,UPA}(x;v_i)$ is the utility of the uniform price auction under bid profile $x$ and valuation $v_i$. Then a player's utility in the game is: $u_i^n(s;v_i)=\E_z[u_i^{n,z}(s;v_i)]$.

We will also use the \emph{extended utility} for the uniform price auction that we defined in Section \ref{sec:intro-uniform}.
\begin{equation}\label{eqn:util-decomp-demand-unc}
U_i^{n,z}(s; v) = U_i^{n,\text{UPA}}(s\cdot z;v)\cdot z_i
\end{equation}
where $U_i^{n,UPA}$ is as defined in Equation \eqref{eqn:util-decomp-uniform}. Then the \emph{extended utility} for the uniform price auction with noisy demand is simply: $U_i^{n}(s;v) = \E_{z}[U_i^{n,z}(s;v)]$.

We will be using the following Lemma of Swinkels \cite{Swinkels2001}:
\begin{lemma}[Swinkels \cite{Swinkels2001}]\label{lem:swinkels-demand}
Let $B(s;x)$ be the random variable that denotes the number of active bids in strategy profile $s$, that are strictly above $x$. Then for any $\epsilon$, there exists a $k^*(\epsilon)<\infty$
such that for any $k>k^*$:
\begin{equation}
\Pr( B(s;x) = k ) \leq \epsilon
\end{equation}
\end{lemma}
\begin{lemma}[Swinkels\cite{Swinkels2001}]\label{lem:swinkels-cdf}
For a bid vector $s$, let $F_{t}(s;b)$ denote the cummulative density function of the $t$-th highest active bid under strategy profile $s$, evaluated at point $b$. Then for any $d>0$ and for any $\epsilon$ there exists a $k^*(\epsilon,h,h')<\infty$ such that for any $k>k^*(\epsilon,d)$:
\begin{equation}
\forall b\in [0,H], \forall h,h'\in \{0\ldots,d\}: \|F_{k-h+1}(s;b)-F_{k-h'+1}(s;b)\|\leq \epsilon
\end{equation}
\end{lemma}

\begin{theorem}
Consider a uniform price auction game where $k(n)$ units of a good are auctioned off to $n$ players via a uniform price auction. If each player
fails to arrive in the auction with probability $\delta$, then the game satisfies the \emph{vanishing effect condition}.
\end{theorem}
\begin{proof}
Fix $n>0$, $s\in [0,H]^n$, $s_j'\in [0,H]$, $b\in [0,H]$ and $v_i\in [0,\bar{v}]$ and for simplicity of notation, let 
\begin{align*}
u_i'(z)=~&U_i^{n,z}(s_j',s_{-j};b,v)\\
u_i(z) =~&U_i^{n,z}(s;b,v)
\end{align*}
where $U_i^{n,z}$ is as defined in Equation \eqref{eqn:util-decomp-demand-unc}. Also let $u_i'=\E_z[u_i'(z)]$ and $u_i=\E_z[u_i(z)]$. To prove the theorem we need to show that for any $s, s_j', b, v_i$: $ \| u_i'- u_i \| \rightarrow 0$ as $n\rightarrow \infty$. In other words, for any $\epsilon>0$, there exists $n^*$ such that for any $n>n^*$, $ \| u_i'- u_i \|<\epsilon$.

Without loss of generality we will assume that $s_j'>s_j$ (as the other case is symmetric). For a fixed arrival vector $z$ denote with $p$, $p'$, the allocation of a bid of $b$ under $s$ and $(s_j',s_{-j})$ respectively and with $\theta_{k+1}$, $\theta_{k+1}'$ the $k+1$-highest arriving bid under $s$ and $(s_j',s_{-j})$ respectively. Then for any arrival vector $z$:
\begin{align*}
p' \leq~& p \text{~~~(probability of winning decreases)}\\
\theta_{k+1}' \geq~& \theta_{k+1} \text{~~~(threshold price increases)}\\
 u_i(z)-u_i'(z) =~& v(p-p') - p \theta_{k+1} + p'\theta_{k+1}' \\
\leq~& v(p-p')-p\theta_{k+1}+p\theta_{k+1}'\\
\leq~& \bar{v}(p-p')+p(\theta_{k+1}'-\theta_{k+1})\leq \bar{v}(p-p')+(\theta_{k+1}'-\theta_{k+1})\\
u_i(z)-u_i'(z) \geq~& -p\theta + p'\theta' \geq -p\theta+p'\theta = \theta(p'-p) \geq -H(p-p')
\end{align*}
Thus to argue that $\|u_i-u_i'\|\leq \epsilon$, we can just argue separately that $\E_z[p-p']\leq \frac{\epsilon}{H}$ and $\E_z[\theta_{k+1}'-\theta_{k+1}]\leq \epsilon$. 

The second part will follow by Lemma \ref{lem:swinkels-cdf}. For any instantiation of $z$ let $\theta_{t}^{-j}$ be the $t$-th highest active bid among all bids except player $j$'s bid. Then $\theta_{k+1}'\leq \theta_{k}^{-j}$ (the $k+1$-highest active bid is at most the $k$-th highest bid excluding player $j$'s bid). Moreover, $\theta_{k+1}\geq \theta_{k+1}^{-j}$. Thus:
\begin{equation}
\E[\theta_{k+1}'-\theta_{k+1}]\leq \E[\theta_{k}^{-j}-\theta_{k+1}^{-j}]
\end{equation}
Now by Lemma \ref{lem:swinkels-cdf} there always exist a market size $n^*(\epsilon)$ such that this difference is at most $\epsilon\cdot H$, since the cummulative density functions of $\theta_{k}^{-j}$ and $\theta_{k+1}^{j}$ differ by at most $\epsilon$ and the variables are bounded in $[0,H]$.
%
%
%For an activeness vector $z$, let $\Delta u_i(z)$ be the utility difference between $s$ and $(s_j',s_{-j})$, $E(z)=|\{k\in [n]: s_k\cdot z_k=b\}|$ be the number of active players who bid $b$ in profile $s$ and with $G(z)=|\{k\in [n]: s_k\cdot z_k>b\}|$ be the number of active players with bid strictly above $b$ and with $L(z)=n-G(z)-E(z)$ be the number active players who bid strictly below $b$. Observe that all three variables are distributed independently, since they depend on the arrival of disjoint sets of players. Moreover, let $n_1$, $n_2$ and $n_3$ be the upper bound on $E(z),G(z)$ and $L(z)$ respectively, i.e. the number of total (not necessarily active) players who bid equal, strictly above or strictly below $b$.
%
%We will show that conditional on any value of $I(z)$ the expected utility difference goes to $0$, i.e. $\E[\Delta u_i | I(z)=p]\rightarrow 0$ for any $p\in \{0,1\}$.
%%\begin{multline*}
%%\E_z[\Delta u_i(z)] =\\ \sum_{p=1}^{n_1} \sum_{q=1}^{n_2} \sum_{r=1}^{n_3} \E_z[\Delta u_i(z) | I(z)=p, G(z)=q, L(z)=r] \Pr[I(z)=p,G(z)=q,L(z)=r]
%%\end{multline*}
%%
%%If $I(z)\geq \frac{\bar{v}}{\epsilon}$, then 
%%\[p(s'\cdot z; b) - p(s\cdot z; b)=\leq \frac{1}{I(z)}\]
%
%If $G(z)\geq  k$, then a bid of $b$ is never allocated, even if player $j$ increases his strategy from $s_j$ to $s_j'$. Thus $\Delta u_i(z)=0$. 
%
%If $G(z)\leq k-1-p$, then a bid of $b$ is always allocated even if player $j$ increases his bid. The only thing that $j$ can affect is the uniform price, i.e. $\Delta u_i(z) = \Delta \theta_{k+1}(z)$. If $G(z)+L(z)=t-p$, then the change in the threshold price is at most $s_{t-1}-s_t$.
%
%If $G(z)\in [k-p,k-1]$, then a switch in the bid of $j$ from $s_j$ to $s_j'>s_j$, can decrease the allocation probability by at most $\frac{1}{p-1}$ if $p>1$ and at most $1$ if $p=1$. The reason is that prior to the change we have: $p(s\cdot z; b) = \frac{k-G(z)}{p}$. After $j$ increases his bid, in the worst case $j$ was a player who was bidding $b$ and hence the allocation probability is $p(s'\cdot z;b) = \frac{k-G(z)-1}{p-1}$ if $p>1$ and $p(s'\cdot z;b)=0$ if $p=1$, leading to a difference of $\|p(s'\cdot z; b) -p(s\cdot z;b)\| \leq \frac{1}{p-1}$ if $p>1$ and $1$ if $p=1$. Thus we also get that $\Delta u_i(z) \leq \frac{\bar{v}}{p-1}$ if $p>1$ and $\Delta u_i(z)\leq \bar{v}$ if $p=1$.
%
%
%\begin{multline*}
%\E_z[\Delta u_i(z) | I(z)=p] =\\ \sum_{q=1}^{k-p-1} \sum_{r=1}^{n_3} \E_z[\Delta u_i(z) | I(z)=p, G(z)=q, L(z)=r] \Pr[G(z)=q,L(z)=r]
%\end{multline*}
% 

Now we move on to proving the first part: $\E_z[p-p']\leq \frac{\epsilon}{H}$. We will condition on the number of active players that have a bid equal to $b$. Let this number be $T$. Also let $n(b)$ the total number of players with bid equal to $b$ in $s$ (active or not). Thus $T\in [0,n(b)]$. Moreover, we will denote with  $b^*$ be the next highest bid after $b$, among all the bids in $s$ including the non-active ones. We will show that conditional on any number $T$ of ties, the expected change in utility of a player is at most $\epsilon$ for some sufficiently large $n>n^*$.

For any $T$, the allocation probability $p(s\cdot z;b)$ can change with the unilateral increase of player $j$ from $s_j$ to $s_j'$ only if the number of players that bid strictly above $b$ is in the range of $[k-T,k-1]$, i.e if $B(s;b)\in [k-T,k-1]$. If $B(s;b)\leq	 k-T-1$, then even if all players with bid $b$ are allocated, there is still one extra unit left. Hence, an increase in the bid of another player $j$ cannot affect the allocation, which is always $1$. If $B(s;b)\geq k$, then the allocation probability is $0$ and an increase in some player's bid can only decrease the allocation probability. 

Moreover, observe that if $B(s;b)\in [k-T+1,k-1]$ then currently the player is tying at the threshold price, which means that $p(s;b)=\frac{k-B(s;b)}{T}$. If the deviating player was among the tying ones, then his deviation can cause the allocation probability to become $\frac{k-B(s;b)-1}{T-1}$, causing a difference of at most $\frac{1}{T-1}$. If he was not, then it can cause the allocation probability to become $\frac{k-B(s;b)-1}{T}$, causing a difference of $\frac{1}{T-1}$. Thus in any of this cases, the allocation difference is at most $\frac{1}{T-1}$. 

If $B(s;b)=k-T$, then currently the player is being deterministically allocated and after the deviation his allocation can drop to $\frac{1}{T}$ if $T>1$ and to $0$ if $T=1$. 

Thus we can write the expected difference as:
\begin{equation}
\sum_{t=1}^{n(b)}\left(\sum_{x=k-t+1}^{k-1} \Pr[B(s;b)=x]\frac{1}{t-1} + \Pr[B(s;b)=k-t]\cdot 1\right)\Pr[T=t]
\end{equation}
We separate this as:
\begin{align*}
I_1 =~& \sum_{t=1}^{n(b)}\left(\sum_{x=k-t+1}^{k-1} \Pr[B(s;b)=x]\frac{1}{t-1}\right) \Pr[T=t]\\
I_2 =~& \sum_{t=1}^{n(b)}\Pr[B(s;b)=k-t]\Pr[T=t]
\end{align*}
Observe that $I_2=\Pr[B(s;b^*)=k]$. Hence, by Lemma \ref{lem:swinkels-demand}, we know that for any $k>k^*\left(\frac{\epsilon}{\bar{v}}\right)$, $I_2\leq \frac{\epsilon}{\bar{v}}$.

Now we argue about $I_1$. Observe that for any $t>\frac{\bar{v}}{\epsilon}+1$:
\begin{equation*}
\sum_{x=k-t+1}^{k-1} \Pr[B(s;b)=x]\frac{1}{t-1}\leq \frac{\epsilon}{\bar{v}}
\end{equation*}
For any $t<\frac{\bar{v}}{\epsilon}$, we know by Lemma \ref{lem:swinkels-demand} that for $k>k^*\left(\frac{\epsilon}{\bar{v}}\right)+\frac{\bar{v}}{\epsilon}>k^*(\epsilon)+t$, we have that: $\Pr(B(s;b)=k-x)\leq \frac{\epsilon}{\bar{v}}$. Thus for $n>n^*$ with $k(n^*)>k^*\left(\frac{\epsilon}{\bar{v}}\right)+\frac{\bar{v}}{\epsilon}$, we have:
\begin{align*}
\sum_{x=k-t+1}^{k-1} \Pr[B(s;b)=x]\frac{1}{t-1}\leq \frac{\epsilon}{\bar{v}}\sum_{x=k-t+1}^{k-1}\frac{1}{t-1}=\frac{\epsilon}{\bar{v}}
\end{align*}
Thus we get that for any $\epsilon$, there exists $n^*(\epsilon)$ such that for any $n>n^*(\epsilon)$, $I_1 \leq \frac{\epsilon}{\bar{v}}$. This completes the Theorem.
\end{proof}

\begin{lemma}
If a mechanism is non-atomic $(\lambda,\mu)$-smooth, then the endogenous noisy demand version of the mechanism where each player fails to arrive independently with probability $\delta$ is also a non-atomic $(\lambda,\mu)$-smooth mechanism. 
\end{lemma}
\begin{proof}
By non-atomic smoothness of the original mechanism we know that for any valuation vector $v$, there exists for each player $i$ a deviation $s_i^*(v)$ such that for any strategy profile $s$:
\begin{equation*}
\sum_{i=1}^{n} U_i^n(s_i^*(v),s_{-i};v_i) \geq \lambda \opt^n(v) - \mu \rev^n(s)
\end{equation*}
Observe that for any strategy profile $s$:
\begin{equation*}
 U_i^n(s_i^*(v\cdot z),s_{-i};v_i)\cdot z_i \geq U_i^n(s_i^*(v\cdot z),s_{-i};v_i\cdot z_i)
\end{equation*}
Observe that:
\begin{align*}
\E_{z,\tilde{z}}\left[U_i^n( s_i^*(v\cdot (z_i,\tilde{z}_{-i})),s_{-i}\cdot z_{-i};v_i)\cdot z_i\right] =~& \E_{z,\tilde{z}}\left[U_i^n(s_i^*(v\cdot \tilde{z}),s_{-i}\cdot z_{-i};v_i)\cdot \tilde{z}_i\right]\\
\geq~&  \E_{z,\tilde{z}}\left[U_i^n(s_i^*(v\cdot \tilde{z}),s_{-i}\cdot z_{-i};v_i\cdot \tilde{z}_i)\right]
\end{align*}

Thus, for any strategy profile $s$, valuation profile $v$ and arrival vector $z$:
\begin{multline*}
\sum_{i\in [n]} \E_{z,\tilde{z}}\left[U_i^n( s_i^*(v\cdot (z_i,\tilde{z}_{-i})),s_{-i}\cdot z_{-i};v_i)\cdot z_i\right]\geq \\
\E_{z,\tilde{z}}\left[\sum_i U_i^n(s_i^*(v\cdot \tilde{z}),s_{-i}\cdot z_{-i};v_i\cdot \tilde{z}_i)\right]\geq \E_{z,\tilde{z}}\left[\lambda \opt^n(v\cdot \tilde{z})-\mu \rev^n(s\cdot z)\right]
\end{multline*}

Observe that: $\E_{\tilde{z}}\left[U_i^n(s_i^*(v\cdot (z_i,\tilde{z}_{-i})),s_{-i}\cdot z_{-i}; v_i)\cdot z_i\right]$ corresponds to the utility of a player under the following deviation: random sample an arrival vector $\tilde{z}_{-i}$, deviate assuming the arrival vector $(z_i,\tilde{z}_{-i})$. This is a valid deviation for the noisy demand mechanism and hence the above inequality shows that the noisy demand mechanism is a non-atomic smooth mechanism.
\end{proof}

==> oldtable.tex <==
\begin{table}
\begin{center}
\begin{tabular}{@{} c @{\hspace{.2cm}} >{\bf}D{.}{.}{3} @{\hspace{.4cm}} D{.}{.\
}{3} @{\hspace{.27cm}} c @{}}
        \hline\noalign{\smallskip}
%                                                                               
                    &                                                    & \mul\
ticolumn{1}{@{\hspace{.3cm}} c}{Atomic} &  \\
                    & \multicolumn{1}{c @{}}{\textbf{Atomic}}       & \multicol\
umn{1}{@{\hspace{.3cm}} c}{unsplittable} &  \\
                Degree & \multicolumn{1}{c @{}}{\textbf{splittable}} & \multico\
lumn{1}{@{\hspace{.3cm}} c}{(weighted) \cite{ADG11a}} & \multicolumn{1}{c @{}}{\
Nonatomic \cite{RT04}} \\
%                                                                               
                \noalign{\smallskip}
                \hline
                \noalign{\smallskip}
        %                                                                       
                1 &   1.\textbf{500} &             2.618 & 1.333 \\
                2 &   2.\textbf{549} &             9.909 & 1.626 \\
                3 &   5.\textbf{063} &            47.82  & 1.896 \\
                4 &  11.\textbf{09 } &           277.0   & 2.151 \\
                5 &  26.\textbf{32 } &       1{,}858     & 2.394 \\
                6 &  66.\textbf{88 } &      14{,}099     & 2.630 \\
                7 & 180.\textbf{3  } &     118{,}926     & 2.858 \\
                8 & 512.\textbf{0  } & 1{,}101{,}126     & 3.081 \\
%                                                                               
                \noalign{\smallskip}
%                                                                               
                $d$ & \multicolumn{1}{c @{\hspace{.05cm}}}{$(\frac{1+\sqrt{d+1}\
}{2})^{d+1}$} & \multicolumn{1}{@{\hspace{.1cm}} c @{}}{$\Theta( \frac{d}{\log \
d} )^{d+1}$} & $\Theta( \frac{d}{\log d} )$ \\
        \noalign{\smallskip}
        \hline
        \end{tabular}
        \caption{The price of anarchy in the special case of
          polynomial cost functions with nonnegative coefficients.  For
        splittable congestion games, the lower bounds are contributed
        by the present work.  The upper bound of~$\tfrac{3}{2}$ for affine cost
        functions was first proved by Cominetti et~al.~\cite{CCS09a}.
        For higher-degree polynomials, we give the first
        closed-form POA upper bounds, essentially matching the
        numerical upper bounds computed by Harks~\cite{H11a}.}\label{tab:Compar\
ison}
\end{center}
\end{table}


==> preliminaries.tex <==
% TEX
In this work, we present a framework to study the efficiency of games in the large.  We apply this framework to a variety of games, including cost minimization games, value maximization games, and welfare maximization in mechanisms.  
For the sake of brevity, we present our framework for cost minimization settings. 
Analogous frameworks exist for the other settings, and we defer their presentation to the corresponding sections. 

A cost minimization game $G^n$ consists of a set $N$ of $n$ players, a type space $T^n=T_1\times\ldots\times T_n$ specifying a set of potential types $T_i$ for each player, a strategy space $S^n=S_1\times\ldots\times S_n$ specifying a set of potential strategies $S_i$ for each player, and a cost function $c_i^n$ for each player.  In an instantiation of the game, each player $i$ has a type $t_i\in T_i$.  The type of a player determines his feasible strategy space $S_i(t_i) \subseteq S_i$.  Write $S(t) = S_1(t_1) \times \ldots\times S_n(t_n)$ for the set of admissible strategy profiles given type profile $t$.  The cost of a player depends on his type and the strategies of all players, $c_i^n:S^n\times T_i\rightarrow\Re$, denoted as $c_i^n(s;t_i)$. The objective is to select an outcome that minimizes the social cost.  
Let $\SC^n(s;t)$ denote the social cost at strategy profile $s$, i.e.,
\begin{equation}
\SC^n(s;t) = \sum_{i=1}^n c_i^n(s; t_i).
\end{equation}
The optimal cost for type profile $t$ will be denoted by $\opt^n(t)$; i.e., 
\begin{equation}
\opt^n(t) = \min_{s\in S^n}\SC^n(s;t)
\end{equation}
%
\iffalse
Similarly, in a cost minimization game, such as a routing game, players have cost functions $c_i^n:S^n\times T_i\rightarrow\Re$, denoted as $c_i^n(s;t_i)$, and the goal is to select an outcome that minimizes total cost.  Thus,
\begin{equation}
\opt^n(t) = \min_{s\in S^n}\sum_{i=1}^n c_i^n(s; t_i)
\end{equation}
and $C^n(s;t)$, the cost at strategy profile $s$, is
\begin{equation}
W^n(s;t) = \sum_{i=1}^n u_i^n(s; t_i).
\end{equation}
Finally, an auction is a game in which agents compete for goods.  The mechanism specifies, for each strategy profile, an allocation $x(s^n)=x_1(s^n)\times\ldots\times x_n(s^n)$ of goods to players and a payment $p(s^n)=p_1(s^n)\times\ldots\times p_n(s^n)$.  The utility function decomposes into a value component, mapping type and allocation to value, and a payment component: $u_i^n(s;t_i)=v_i(x_i(s^n);t_i)-p_i(s^n)$.  In this case, the goal is to select an allocation that maximizes total value, i.e.,
\begin{equation}
\opt^n(t) = \max_{s\in S^n}\sum_{i=1}^n u_i^n(s; t_i)
\end{equation}
and with $W^n(s;t)$ the welfare at strategy profile $s$, i.e.,
\begin{equation}
W^n(s;t) = \sum_{i=1}^n u_i^n(s; t_i).
\end{equation}
And revenue is blah.
\fi
%

%%\subsection{Equilibria and the Price of Anarchy}

For a fixed game $G^n$, we can imagine a Bayesian setting in which player types are drawn independently from distributions; that is, for each player $i$ there is a distribution $\F_i$ over $T_i$, and we think of $t_i$ as being drawn independently from $\F_i$.  A strategy function for agent $i$ is a (possibly randomized) mapping from $T_i$ to $S_i$, which we think of as a specification of the action to use given a type.  A $\BCCE$ is a profile of strategy functions such that no single agent can decrease her expected cost (over randomization in types and strategies) by unilaterally modifying her strategy.  Formally, the profile of strategy functions $s$ is a $\BCCE$ if for all $i$, all types $t_i$, and all alternative strategies $s_i' \in S_i$, we have
\[ \E_{t_{-i} \sim \F_{-i}}[c_i^n(s_i(t_i), s_{-i}(t_{-i});t_i)] \leq \E_{t_{-i} \sim \F_{-i}}[c_i^n(s_i', s_{-i}(t_{-i});t_i)]. \]
Note that the non-Bayesian notion of Nash Equilibrium is a special case of the above, in which every distribution $\F_i$ is a point mass.

The Price of Anarchy (PoA) of game $G^n$ is the worst-case ratio between the expected optimal cost and the expected social cost at equilibrium, over all type distributions and all $\BCCE$. Formally, the Bayes-Nash Price of Anarchy of a game $G^n$ is 
\[ \BCCE\mbox{-}\poa^n = \max_{\F} \max_{s}\frac{\E_{t \sim \F}[\SC^n(s(t);t)]}{\E_{t \sim \F}[\opt^n(t)]} \]
where the maximum over strategies $s$ is taken over all $\BCCE$ for distribution profile $\F$. 

==> simultaneous-lower-bound.tex <==
% !TEX root=large.tex
\subsection{Constant Inefficiency in the Limit under Supply Uncertainty}

In the previous section we showed that noisy arrival of players leads to full efficiency in the limit.
Here we show that this ''demand uncertainty" was, in some sense, the ''right" type of uncertainty.
In particular, other types of uncertainty that have proved useful in the literature fail to achieve efficiency for simultaneous uniform price auctions.
For example, Swinkels \cite{Swinkels2002} has considered supply uncertainty (rather than demand uncertainty), namely that the probability that the number of units of the good equals to any fixed number goes to $0$ as the market grows large.
Swinkels showed that for a uniform price auction of a single good with decreasing marginal valuations, this source of inefficiency is sufficient to recover full efficiency in the limit. 
In contrast, we show that for simultaneous uniform price auctions, this form of supply uncertainty can lead to a constant factor inefficiency even in the limit. In particular, it sustains a ``search friction'' in the limit: players do not know which items will have higher supply and thereby cannot decide which items to target. At equilibrium, their prediction of which items are the right to target ends up leading to constant factor inefficiencies that do not vanish.
%
%However, in a single uniform price auction there are no search frictions and the players don't face a problem of having to pick which %items they want to target. 

It is worthwhile to mention that Swinkels' result, for the case of a single good with decreasing marginal values, can be derived using our framework as well.
The smoothness deviation in this case is simply to report the true values. 
Such smoothness deviations that are independent of the supply of goods imply full efficiency under supply uncertainty. 
However, in the case of simultaneous uniform price auctions the supply affects the optimal allocation of a player, which in turn determines the smoothness deviation. 
A concrete counter example showing that the supply uncertainty used in \cite{Swinkels2002} may lead to constant inefficiency in simultaneous uniform price auctions appears as Example \ref{ex:inefficiency-supply} in Appendix \ref{sec:uniform-app}.







